Improving Lagarias-Odlyzko Algorithm For Average-Case Subset Sum: Modular Arithmetic Approach

Lagarias and Odlyzko (J.~ACM~1985) proposed a polynomial time algorithm for solving ``\emph{almost all}'' instances of the Subset Sum problem with $n$ integers of size $\Omega(\Gamma_{\text{LO}})$, where $\log_2(\Gamma_{\text{LO}}) > n^2 \log_2(\gamma)$ and $\gamma$ is a parameter of the lattice basis reduction ($\gamma > \sqrt{4/3}$ for LLL). The algorithm of Lagarias and Odlyzko is a cornerstone result in cryptography. However, the theoretical guarantee on the density of feasible instances has remained unimproved for almost 40 years. In this paper, we propose an algorithm to solve ``almost all'' instances of Subset Sum with integers of size $\Omega(\sqrt{\Gamma_{\text{LO}}})$ after a single call to the lattice reduction. Additionally, our argument allows us to solve the Subset Sum problem for multiple targets while the previous approach could only answer one target per call to lattice basis reduction. We introduce a modular arithmetic approach to the Subset Sum problem. The idea is to use the lattice reduction to solve a linear system modulo a suitably large prime. We show that density guarantees can be improved, by analysing the lengths of the LLL reduced basis vectors, of both the primal and the dual lattices simultaneously.

==> Makefile <==
SOURCES := $(shell find $(SOURCEDIR) -name '*.tex')

all: main.pdf

main.pdf: $(SOURCES) main.bbl 
	pdflatex main.tex
	pdflatex main.tex

main.aux: $(SOURCES)
	pdflatex main.tex

main.bbl: bib.bib main.aux
	bibtex main

clean:
	rm -f img/*.log img/*.aux 
	rm -f *~ *.log *.out *.aux *.blg *.bbl *.gz

distclean: clean
	rm -f main.pdf

tar: clean
	bash -c "cd ..; tar -czf ${BASE}.tar.gz ${BASE}/*; mv ${BASE}.tar.gz ${BASE}"

spell:
	@for i in `find . -name "*.tex"` ; do \
		echo "------------ $$i --------------" ; \
		aspell list --lang=en --mode=tex --dont-tex-check-comments --personal=./blue-slownik.txt < $$i | sort | uniq ; \
done

diff:
	mkdir /tmp/cut-and-count-diff/
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d2.tex
	git checkout $(branch-id)
	python2 ~/latex-flatten.py main.tex /tmp/cut-and-count-diff/test.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test.tex /tmp/cut-and-count-diff/test2.tex
	python2 ~/latex-flatten.py /tmp/cut-and-count-diff/test2.tex /tmp/cut-and-count-diff/d1.tex
	latexdiff /tmp/cut-and-count-diff/d1.tex /tmp/cut-and-count-diff/d2.tex > /tmp/cut-and-count-diff/diff.tex
	pdflatex /tmp/cut-and-count-diff/diff.tex
	git checkout master


==> chapters/babai.tex <==
\newcommand{\LO}{\textsf{LO}}
\newcommand{\rvline}{\hspace*{-\arraycolsep}\vline\hspace*{-\arraycolsep}}

\section{Truncated Lagarias-Odlyzko\label{sec:Babai}}


In this section, we show that our analysis allows us to improve the guarantees
on Lagarias-Odlyzko lattice. In this section, we present the algorithm which we call \emph{Truncated
Lagarias-Odlyzko} algorithm (Truncated LO). This algorithm will be a slight
modification of the original Lagarias-Odlyzko procedure, with a small caveat that we
interrupt it at the last step of LLL.

\karol{Define what is $K$}

For an instance of Subset Sum $a_1,\ldots,a_n$ with target value $T$, consider a
reordered variant of the Lagarias-Odlyzko lattice
\begin{displaymath}
    \LO(a_1,\ldots,a_n,T) \coloneqq
    \left(
\begin{array}{ccccc|c}
    K a_1 & K a_2 & K a_3 & \cdots & K a_n & - K T\\
    \hline
    1 & 0 & 0 & \cdots & 0 & 0\\
    0 & 1 & 0 & & 0 & 0 \\
    0 & 0 & 1 & & 0 & 0\\
    \vdots & \vdots &\vdots & \ddots  & \vdots & \vdots \\
    0 & 0 & 0 &\ldots & 1 & 0 
\end{array}\right) \in \mathbb{Z}^{(n+1) \times (n+1)}.
\end{displaymath}
Instead of running LLL on the full lattice, we propose the following
strategy. First, we run LLL on the truncated lattice:
\begin{displaymath}
    \LO_{\textsf{tr}}(a_1,\ldots,a_n) \coloneqq
    \left(
    \begin{array}{ccccc}
    K a_1 & K a_2 & K a_3 & \cdots & K a_n \\
    \hline
    1 & 0 & 0 & \cdots & 0 \\
    0 & 1 & 0 & & 0  \\
    0 & 0 & 1 & & 0 \\
    \vdots & \vdots &\vdots & \ddots  & \vdots \\
    0 & 0 & 0 &\ldots & 1 
    \end{array}\right) \in \mathbb{Z}^{(n+1) \times n)}
\end{displaymath}
This returns us the basis $b_1,\ldots,b_n$. Next, we  apply Babai's nearest
plane algorithm on this LLL-reduced basis to find a vector $\V{r}$ in
$\LO_{\textsf{tr}}$ close to $\V{q} = (-KT,0,0,\cdots,0)^\trans$. Finally, the
\emph{Truncated LO} algorithm terminates and returns vector
$\V{r}$. This concludes the description of the procedure.

We remark that the above sequence of operations is the same as the initial segment of the
operations that would be performed when applying LLL on the full
Lagarias-Odlyzko lattice $\LO(a_1,\ldots,a_n,T).$ We just interrupt procedure
before the final basis swapping of LLL. As a consequence, this
procedure is slightly faster than the Lagarias-Odlyzko algorithm.
  
Now, we prove a tighter bound on our modified algorithm compared to
the initial Lagarias-Odlyzko bound. More precisely:

\begin{theorem}\label{thm:babai}
    Let $a_1,\ldots,a_n \in \mathbb{Z}$ be integers drawn uniformly at random
    from the range $\{1,\ldots,R\}$, where $R \coloneqq \Theta(\gamma^{n^2/2 + 8
    n \log(n)})$.  Let $T$ be an arbitrary integer.

    Then,  with probability $\ge 1-2^{-\Omega(n \log{n})}$ the Truncated LO
    algorithm on $\LO(a_1,\ldots,a_n,T)$ returns a vector $(K T
    ,e_1,\ldots,e_n)^\trans \in \{0,1\}^n$ with $\sum_{i=1}^n e_i a_i = T$ and
    $\sum_{i=1}^n e_i \le n/2$ if it exists.
\end{theorem}



By arguments from the previous section we have the following inequality:

\begin{proposition}\label{prop:babai-inequality}
    For all $i \in \{1,\ldots,n\}$ it holds that:
    \begin{displaymath}
        \prob{\norm{\V{b}_i^\ast} \ge \sqrt{2n}} \ge 1-2^{-\Omega(n \log{n})}.
    \end{displaymath}
\end{proposition}

The proof of~\cref{prop:babai-inequality} is analogous to the proof
of~\cref{lem:main-bound} and we postpone it
to~\cref{sec:proof-babai-inequality}. The final step of our procedure is to
invoke Babai's nearest plane algorithm. We use the following property of the
Babai's nearest plane algorithm.

\todo{Citation needed}
\begin{lemma}[Babai's Nearest Plane]\label{lem:babai}
    For given basis $\V{b}_1,\ldots,\V{b}_n \in \mathbb{Z}^{m}$ and
    a vector $\V{q} \in \mathbb{Z}^{m}$, Babai's nearest plane algorithm
    returns vector $\V{r} \in \mathbb{Z}^{m}$ such that:
    \begin{enumerate}[label=(\roman*)]
        \item\label{it:p1} $\V{r} \in \mathrm{span}(\V{b}_1^\ast,\ldots,\V{b}_n^\ast)$, and
        \item\label{it:p2} $\dotprod{ \V{q} - \V{r}, \V{b}_i^\ast } \le
            \frac{1}{2} \cdot \norm{\V{b}_i^\ast}^2$.
    \end{enumerate}
    Such a vector $\V{r}$ always exists. Furthermore, if $\dotprod{\V{q} -
    \V{r}, \V{b}^\ast_i} < \frac{1}{2} \norm{\V{b}_i^\ast}^2$
    for all $i \in \{1,\ldots,n\}$, then the vector $\V{r}$ is \emph{unique}.
\end{lemma}

% Observe for us it holds that $\V{b}_n = (K,0,\ldots,0)^\trans$, because invoking
% Babai's algorithm on $\V{q} = (-KT,0,\ldots,0)^\trans$ for $b_1,\ldots,b_n$ is identical
% to invoking Babai's algorithm on $(0,T\cdot \V{v})$ for basis
% $b_1,\ldots,b_{n-1}$.

Consider a vector $\V{e} = (K T,e_1,\ldots,e_n)^\trans$ such that $e_i \in
\{0,1\}$ for all $i \in \{1,\ldots,n\}$, $\sum_{i=1}^n
e_i \cdot a_i = T$ and $\sum_{i=1}^n \le n/2$. Observe, that
$\V{e} \in \LO_{\text{tr}}(a_1,\ldots,a_n)$, and hence $\V{e} \in
\mathrm{span}(b_1,\ldots,b_n)$. Moreover, by~\cref{prop:babai-inequality} we have that
\begin{displaymath}
    \dotprod{ \V{e} - \V{q} , \V{b}_i} \le \norm{(0,e_1,\ldots,e_n)}  \cdot \norm{\V{b}_i} \le
    \sqrt{n/2} \cdot \norm{\V{b}_i} < \frac{1}{2} \norm{\V{b}_i}^2.
\end{displaymath}

Therefore, vector $\V{e}$ satisfies the properties~\ref{it:p1} and \ref{it:p2}
of~\cref{lem:babai}. Note, that property~\ref{it:p2} is satisfied with sharp
inequality. Therefore, Babai's nearest plane algorithm returns a vector uniquely
defined by those properties. Since $\V{e}$ also satisfies these properties, it
means that Babai's nearest plane algorithm actually returns vector $\V{e}$.

